Measuring the Impact of Lexical Training Data Coverage on Hallucination Detection in Large Language Models

Hallucination in large language models (LLMs) is a fundamental challenge, particularly in open-domain question answering. Prior work attempts to detect hallucination with model-internal signals such as token-level entropy or generation consistency, while the connection between pretraining data exposure and hallucination is underexplored. Existing studies show that LLMs underperform on long-tail knowledge, i.e., the accuracy of the generated answer drops for the ground-truth entities that are rare in pretraining. However, examining whether data coverage itself can serve as a detection signal is overlooked. We propose a complementary question: Does lexical training-data coverage of the question and/or generated answer provide additional signal for hallucination detection? To investigate this, we construct scalable suffix arrays over RedPajama's 1.3-trillion-token pretraining corpus to retrieve $n$-gram statistics for both prompts and model generations. We evaluate their effectiveness for hallucination detection across three QA benchmarks. Our observations show that while occurrence-based features are weak predictors when used alone, they yield modest gains when combined with log-probabilities, particularly on datasets with higher intrinsic model uncertainty. These findings suggest that lexical coverage features provide a complementary signal for hallucination detection. All code and suffix-array infrastructure are provided at https://github.com/WWWonderer/ostd.

==> table_3b_rougeL.tex <==
\begin{table*}[!t]
\centering
\small
\begin{tabular}{@{}lllc@{\hskip 6pt}cc|@{\hskip 6pt}cc@{}}
\toprule
\textbf{Feature Type} & \textbf{Dataset} & \textbf{Model} & \textbf{Tree Depth} & \textbf{Train Acc (Log)} & \textbf{Train Acc (Full)} & \textbf{Test Acc (Log)} & \textbf{Test Acc (Full)} \\
\midrule

\multirow{22}{*}{\textbf{Raw Freq}} & \multirow{7}{*}{TriviaQA} & \multirow{6}{*}{Tree}
& 3  & 0.736 $\pm$ 0.004 & \textbf{0.746} $\pm$ 0.004 & 0.736 $\pm$ 0.011 & \textbf{0.749} $\pm$ 0.008 \\
& & & 5  & 0.742 $\pm$ 0.003 & \textbf{0.760} $\pm$ 0.005 & 0.730 $\pm$ 0.013 & \textbf{0.736} $\pm$ 0.013 \\
& & & 7  & 0.756 $\pm$ 0.005 & \textbf{0.788} $\pm$ 0.012 & 0.726 $\pm$ 0.005 & \textbf{0.732} $\pm$ 0.017 \\
& & & 9  & 0.776 $\pm$ 0.006 & \textbf{0.829} $\pm$ 0.011 & 0.714 $\pm$ 0.003 & \textbf{0.715} $\pm$ 0.015 \\
& & & 10 & 0.787 $\pm$ 0.007 & \textbf{0.855} $\pm$ 0.011 & \textbf{0.718} $\pm$ 0.011 & 0.709 $\pm$ 0.013 \\
& & & 20 & 0.913 $\pm$ 0.008 & \textbf{0.992} $\pm$ 0.004 & 0.673 $\pm$ 0.022 & \textbf{0.678} $\pm$ 0.027 \\
& & NN & -- & 0.733 $\pm$ 0.001 & \textbf{0.736} $\pm$ 0.002 & \textbf{0.740} $\pm$ 0.007 & 0.737 $\pm$ 0.007 \\

\addlinespace


& \multirow{7}{*}{NQ-Open} & \multirow{6}{*}{Tree}
& 3  & 0.613 $\pm$ 0.007 & \textbf{0.628} $\pm$ 0.014 & 0.529 $\pm$ 0.030 & \textbf{0.551} $\pm$ 0.037 \\
& & & 5  & 0.639 $\pm$ 0.010 & \textbf{0.695} $\pm$ 0.004 & 0.514 $\pm$ 0.028 & \textbf{0.559} $\pm$ 0.037 \\
& & & 7  & 0.670 $\pm$ 0.015 & \textbf{0.770} $\pm$ 0.018 & 0.516 $\pm$ 0.036 & \textbf{0.548} $\pm$ 0.048 \\
& & & 9  & 0.702 $\pm$ 0.024 & \textbf{0.835} $\pm$ 0.024 & 0.516 $\pm$ 0.028 & \textbf{0.548} $\pm$ 0.044 \\
& & & 10 & 0.715 $\pm$ 0.030 & \textbf{0.868} $\pm$ 0.034 & 0.519 $\pm$ 0.030 & \textbf{0.541} $\pm$ 0.043 \\
& & & 20 & 0.849 $\pm$ 0.044 & \textbf{1.000} $\pm$ 0.000 & 0.484 $\pm$ 0.047 & \textbf{0.544} $\pm$ 0.042 \\
& & NN & -- & 0.580 $\pm$ 0.009 & \textbf{0.582} $\pm$ 0.003 & \textbf{0.567} $\pm$ 0.023 & 0.544 $\pm$ 0.021 \\

\addlinespace

& \multirow{7}{*}{CoQA} & \multirow{6}{*}{Tree}
& 3  & 0.666 $\pm$ 0.004 & \textbf{0.668} $\pm$ 0.007 & \textbf{0.668} $\pm$ 0.017 & 0.664 $\pm$ 0.011 \\
& & & 5  & 0.671 $\pm$ 0.004 & \textbf{0.678} $\pm$ 0.004 & \textbf{0.669} $\pm$ 0.016 & 0.667 $\pm$ 0.017 \\
& & & 7  & 0.678 $\pm$ 0.005 & \textbf{0.700} $\pm$ 0.008 & \textbf{0.658} $\pm$ 0.016 & 0.651 $\pm$ 0.017 \\
& & & 9  & 0.689 $\pm$ 0.007 & \textbf{0.735} $\pm$ 0.013 & \textbf{0.654} $\pm$ 0.019 & 0.639 $\pm$ 0.012 \\
& & & 10 & 0.696 $\pm$ 0.007 & \textbf{0.756} $\pm$ 0.016 & \textbf{0.648} $\pm$ 0.020 & 0.633 $\pm$ 0.015 \\
& & & 20 & 0.801 $\pm$ 0.020 & \textbf{0.952} $\pm$ 0.013 & \textbf{0.613} $\pm$ 0.019 & 0.588 $\pm$ 0.012 \\
& & NN & -- & 0.664 $\pm$ 0.004 & \textbf{0.666} $\pm$ 0.004 & \textbf{0.668} $\pm$ 0.013 & 0.665 $\pm$ 0.016 \\

\midrule

\multirow{22}{*}{\textbf{N-gram}} & \multirow{7}{*}{TriviaQA} & \multirow{6}{*}{Tree}
& 3  & 0.738 $\pm$ 0.003 & \textbf{0.741} $\pm$ 0.005 & 0.720 $\pm$ 0.016 & \textbf{0.724} $\pm$ 0.011 \\
& & & 5  & 0.747 $\pm$ 0.004 & \textbf{0.763} $\pm$ 0.004 & \textbf{0.717} $\pm$ 0.021 & 0.712 $\pm$ 0.018 \\
& & & 7  & 0.760 $\pm$ 0.004 & \textbf{0.793} $\pm$ 0.006 & \textbf{0.716} $\pm$ 0.015 & 0.701 $\pm$ 0.011 \\
& & & 9  & 0.780 $\pm$ 0.004 & \textbf{0.836} $\pm$ 0.009 & \textbf{0.705} $\pm$ 0.019 & 0.686 $\pm$ 0.015 \\
& & & 10 & 0.792 $\pm$ 0.004 & \textbf{0.862} $\pm$ 0.007 & \textbf{0.692} $\pm$ 0.021 & 0.683 $\pm$ 0.010 \\
& & & 20 & 0.923 $\pm$ 0.011 & \textbf{0.993} $\pm$ 0.005 & \textbf{0.664} $\pm$ 0.017 & 0.651 $\pm$ 0.014 \\
& & NN & -- & 0.735 $\pm$ 0.004 & \textbf{0.737} $\pm$ 0.003 & \textbf{0.730} $\pm$ 0.012 & 0.728 $\pm$ 0.012 \\

\addlinespace 

& \multirow{7}{*}{NQ-Open} & \multirow{6}{*}{Tree}
& 3  & 0.605 $\pm$ 0.011 & \textbf{0.620} $\pm$ 0.005 & \textbf{0.602} $\pm$ 0.032 & 0.528 $\pm$ 0.030 \\
& & & 5  & 0.622 $\pm$ 0.009 & \textbf{0.690} $\pm$ 0.015 & 0.586 $\pm$ 0.021 & \textbf{0.609} $\pm$ 0.046 \\
& & & 7  & 0.643 $\pm$ 0.016 & \textbf{0.748} $\pm$ 0.019 & \textbf{0.576} $\pm$ 0.027 & 0.566 $\pm$ 0.036 \\
& & & 9  & 0.668 $\pm$ 0.026 & \textbf{0.803} $\pm$ 0.026 & \textbf{0.585} $\pm$ 0.021 & 0.583 $\pm$ 0.053 \\
& & & 10 & 0.680 $\pm$ 0.026 & \textbf{0.833} $\pm$ 0.028 & \textbf{0.591} $\pm$ 0.033 & 0.583 $\pm$ 0.041 \\
& & & 20 & 0.793 $\pm$ 0.048 & \textbf{0.986} $\pm$ 0.016 & 0.548 $\pm$ 0.039 & \textbf{0.555} $\pm$ 0.029 \\
& & NN & -- & 0.586 $\pm$ 0.008 & \textbf{0.601} $\pm$ 0.012 & \textbf{0.590} $\pm$ 0.018 & 0.576 $\pm$ 0.034 \\

\addlinespace

& \multirow{7}{*}{CoQA} & \multirow{6}{*}{Tree}
& 3  & 0.668 $\pm$ 0.002 & \textbf{0.671} $\pm$ 0.006 & 0.661 $\pm$ 0.009 & \textbf{0.666} $\pm$ 0.012 \\
& & & 5  & 0.674 $\pm$ 0.001 & \textbf{0.685} $\pm$ 0.005 & 0.664 $\pm$ 0.004 & \textbf{0.673} $\pm$ 0.010 \\
& & & 7  & 0.686 $\pm$ 0.003 & \textbf{0.711} $\pm$ 0.006 & \textbf{0.663} $\pm$ 0.006 & 0.653 $\pm$ 0.006 \\
& & & 9  & 0.701 $\pm$ 0.004 & \textbf{0.750} $\pm$ 0.010 & \textbf{0.655} $\pm$ 0.006 & 0.642 $\pm$ 0.016 \\
& & & 10 & 0.712 $\pm$ 0.004 & \textbf{0.774} $\pm$ 0.012 & \textbf{0.653} $\pm$ 0.008 & 0.630 $\pm$ 0.020 \\
& & & 20 & 0.827 $\pm$ 0.015 & \textbf{0.962} $\pm$ 0.018 & \textbf{0.627} $\pm$ 0.013 & 0.598 $\pm$ 0.005 \\
& & NN & -- & 0.666 $\pm$ 0.003 & \textbf{0.672} $\pm$ 0.005 & 0.666 $\pm$ 0.010 & \textbf{0.673} $\pm$ 0.008 \\


\bottomrule
\end{tabular}
\caption{Accuracy across tree depths, datasets, and feature types. Bold indicates higher accuracy between log-only and full features. Model: RedPajama-INCITE-3B; metric: ROUGE-L.}
\label{tab:classifier-results-3b}
\end{table*}


==> table_7b_em.tex <==

\begin{table*}[!t]
\centering
\small
\begin{tabular}{@{}lllc@{\hskip 6pt}cc|@{\hskip 6pt}cc@{}}
\toprule
\textbf{Feature Type} & \textbf{Dataset} & \textbf{Model} & \textbf{Tree Depth} & \textbf{Train Acc (Log)} & \textbf{Train Acc (Full)} & \textbf{Test Acc (Log)} & \textbf{Test Acc (Full)} \\
\midrule

\multirow{22}{*}{\textbf{Raw Freq}} & \multirow{7}{*}{TriviaQA} & \multirow{6}{*}{Tree}
& 3  & 0.775 $\pm$ 0.002 & \textbf{0.784} $\pm$ 0.002 & 0.779 $\pm$ 0.008 & 0.779 $\pm$ 0.010 \\
& & & 5  & 0.784 $\pm$ 0.005 & \textbf{0.807} $\pm$ 0.004 & 0.777 $\pm$ 0.016 & \textbf{0.782} $\pm$ 0.009 \\
& & & 7  & 0.799 $\pm$ 0.004 & \textbf{0.837} $\pm$ 0.005 & 0.770 $\pm$ 0.012 & \textbf{0.772} $\pm$ 0.013 \\
& & & 9  & 0.818 $\pm$ 0.006 & \textbf{0.879} $\pm$ 0.009 & 0.765 $\pm$ 0.016 & 0.765 $\pm$ 0.017 \\
& & & 10 & 0.829 $\pm$ 0.008 & \textbf{0.900} $\pm$ 0.009 & \textbf{0.762} $\pm$ 0.011 & 0.759 $\pm$ 0.023 \\
& & & 20 & 0.934 $\pm$ 0.011 & \textbf{0.997} $\pm$ 0.003 & \textbf{0.730} $\pm$ 0.015 & 0.724 $\pm$ 0.019 \\
& & NN & -- & 0.773 $\pm$ 0.002 & \textbf{0.775} $\pm$ 0.005 & \textbf{0.777} $\pm$ 0.009 & 0.776 $\pm$ 0.010 \\

\addlinespace

& \multirow{7}{*}{NQ-Open} & \multirow{6}{*}{Tree}
& 3  & 0.656 $\pm$ 0.021 & \textbf{0.797} $\pm$ 0.018 & 0.600 $\pm$ 0.059 & \textbf{0.730} $\pm$ 0.054 \\
& & & 5  & 0.708 $\pm$ 0.014 & \textbf{0.879} $\pm$ 0.027 & 0.589 $\pm$ 0.048 & \textbf{0.719} $\pm$ 0.031 \\
& & & 7  & 0.771 $\pm$ 0.025 & \textbf{0.947} $\pm$ 0.003 & 0.600 $\pm$ 0.084 & \textbf{0.735} $\pm$ 0.048 \\
& & & 9  & 0.834 $\pm$ 0.030 & \textbf{0.978} $\pm$ 0.008 & 0.584 $\pm$ 0.087 & \textbf{0.746} $\pm$ 0.031 \\
& & & 10 & 0.860 $\pm$ 0.028 & \textbf{0.985} $\pm$ 0.012 & 0.595 $\pm$ 0.069 & \textbf{0.724} $\pm$ 0.030 \\
& & & 20 & 0.958 $\pm$ 0.023 & \textbf{1.000} $\pm$ 0.000 & 0.611 $\pm$ 0.031 & \textbf{0.703} $\pm$ 0.051 \\
& & NN & -- & 0.596 $\pm$ 0.016 & \textbf{0.615} $\pm$ 0.011 & \textbf{0.627} $\pm$ 0.082 & 0.600 $\pm$ 0.055 \\

\addlinespace

& \multirow{7}{*}{CoQA} & \multirow{6}{*}{Tree}
& 3  & 0.647 $\pm$ 0.004 & \textbf{0.706} $\pm$ 0.005 & 0.645 $\pm$ 0.014 & \textbf{0.694} $\pm$ 0.009\\
& & & 5  & 0.652 $\pm$ 0.004 & \textbf{0.739} $\pm$ 0.005 & 0.639 $\pm$ 0.012 & \textbf{0.710} $\pm$ 0.014\\
& & & 7  & 0.659 $\pm$ 0.006 & \textbf{0.767} $\pm$ 0.002 & 0.636 $\pm$ 0.019 & \textbf{0.705} $\pm$ 0.013\\
& & & 9  & 0.670 $\pm$ 0.008 & \textbf{0.806} $\pm$ 0.005 & 0.636 $\pm$ 0.009 & \textbf{0.687} $\pm$ 0.013\\
& & & 10 & 0.676 $\pm$ 0.009 & \textbf{0.831} $\pm$ 0.004 & 0.634 $\pm$ 0.006 & \textbf{0.679} $\pm$ 0.009\\
& & & 20 & 0.777 $\pm$ 0.010 & \textbf{0.991} $\pm$ 0.003 & 0.626 $\pm$ 0.011 & \textbf{0.629} $\pm$ 0.013\\
& & NN & -- & 0.636 $\pm$ 0.004 & \textbf{0.688} $\pm$ 0.005 & 0.639 $\pm$ 0.012 & \textbf{0.687} $\pm$ 0.009\\

\midrule

\multirow{22}{*}{\textbf{N-gram}} & \multirow{7}{*}{TriviaQA} & \multirow{6}{*}{Tree}
& 3  & 0.787 $\pm$ 0.004 & \textbf{0.790} $\pm$ 0.002 & \textbf{0.773} $\pm$ 0.026 & 0.772 $\pm$ 0.025 \\
& & & 5  & 0.799 $\pm$ 0.005 & \textbf{0.808} $\pm$ 0.005 & \textbf{0.766} $\pm$ 0.017 & 0.761 $\pm$ 0.034 \\
& & & 7  & 0.810 $\pm$ 0.005 & \textbf{0.835} $\pm$ 0.006 & 0.758 $\pm$ 0.017 & \textbf{0.759} $\pm$ 0.025 \\
& & & 9  & 0.830 $\pm$ 0.008 & \textbf{0.873} $\pm$ 0.009 & \textbf{0.757} $\pm$ 0.022 & 0.752 $\pm$ 0.024 \\
& & & 10 & 0.842 $\pm$ 0.009 & \textbf{0.891} $\pm$ 0.012 & \textbf{0.756} $\pm$ 0.029 & 0.747 $\pm$ 0.022 \\
& & & 20 & 0.945 $\pm$ 0.019 & \textbf{0.993} $\pm$ 0.004 & \textbf{0.725} $\pm$ 0.027 & 0.719 $\pm$ 0.017 \\
& & NN & -- & 0.786 $\pm$ 0.004 & \textbf{0.788} $\pm$ 0.006 & \textbf{0.776} $\pm$ 0.023 & 0.771 $\pm$ 0.016 \\

\addlinespace

& \multirow{7}{*}{NQ-Open} & \multirow{6}{*}{Tree}
& 3  & 0.668 $\pm$ 0.020 & \textbf{0.770} $\pm$ 0.021 & \textbf{0.588} $\pm$ 0.076 & 0.552 $\pm$ 0.141 \\
& & & 5  & 0.726 $\pm$ 0.029 & \textbf{0.874} $\pm$ 0.036 & 0.600 $\pm$ 0.072 & \textbf{0.612} $\pm$ 0.135 \\
& & & 7  & 0.806 $\pm$ 0.032 & \textbf{0.939} $\pm$ 0.046 & 0.552 $\pm$ 0.089 & \textbf{0.612} $\pm$ 0.112 \\
& & & 9  & 0.859 $\pm$ 0.028 & \textbf{0.977} $\pm$ 0.027 & 0.552 $\pm$ 0.076 & \textbf{0.618} $\pm$ 0.106 \\
& & & 10 & 0.870 $\pm$ 0.032 & \textbf{0.991} $\pm$ 0.016 & 0.570 $\pm$ 0.087 & \textbf{0.594} $\pm$ 0.137 \\
& & & 20 & 0.965 $\pm$ 0.014 & \textbf{1.000} $\pm$ 0.000 & 0.570 $\pm$ 0.112 & \textbf{0.594} $\pm$ 0.143 \\
& & NN & -- & 0.615 $\pm$ 0.053 & \textbf{0.623} $\pm$ 0.048 & 0.546 $\pm$ 0.111 & \textbf{0.582} $\pm$ 0.136 \\

\addlinespace

& \multirow{7}{*}{CoQA} & \multirow{6}{*}{Tree}
& 3  & 0.718 $\pm$ 0.006 & \textbf{0.724} $\pm$ 0.005 & 0.712 $\pm$ 0.012 & 0.712 $\pm$ 0.008 \\
& & & 5  & 0.725 $\pm$ 0.004 & \textbf{0.746} $\pm$ 0.008 & 0.709 $\pm$ 0.012 & \textbf{0.720} $\pm$ 0.015 \\
& & & 7  & 0.736 $\pm$ 0.006 & \textbf{0.784} $\pm$ 0.009 & 0.701 $\pm$ 0.020 & \textbf{0.708} $\pm$ 0.017 \\
& & & 9  & 0.751 $\pm$ 0.009 & \textbf{0.827} $\pm$ 0.011 & \textbf{0.702} $\pm$ 0.019 & 0.694 $\pm$ 0.005 \\
& & & 10 & 0.760 $\pm$ 0.010 & \textbf{0.849} $\pm$ 0.013 & \textbf{0.694} $\pm$ 0.020 & 0.691 $\pm$ 0.012 \\
& & & 20 & 0.864 $\pm$ 0.010 & \textbf{0.985} $\pm$ 0.009 & \textbf{0.677} $\pm$ 0.006 & 0.648 $\pm$ 0.008 \\
& & NN & -- & 0.711 $\pm$ 0.003 & \textbf{0.721} $\pm$ 0.003 & 0.707 $\pm$ 0.013 & \textbf{0.714} $\pm$ 0.012 \\


\bottomrule
\end{tabular}
\caption{Accuracy across tree depths, datasets, and feature types. Bold indicates higher accuracy between log-only and full features. Model: RedPajama-INCITE-7B; metric: EM.}
\label{tab:classifier-results-em}
\end{table*}


==> table_7b_rougeL.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{@{}lllc@{\hskip 6pt}cc|@{\hskip 6pt}cc@{}}
\toprule
\textbf{Feature Type} & \textbf{Dataset} & \textbf{Model} & \textbf{Tree Depth} & \textbf{Train Acc (Log)} & \textbf{Train Acc (Full)} & \textbf{Test Acc (Log)} & \textbf{Test Acc (Full)} \\
\midrule

\multirow{22}{*}{\textbf{Raw Freq}} & \multirow{7}{*}{TriviaQA} & \multirow{6}{*}{Tree} & 3  & 0.747 $\pm$ 0.003 & \textbf{0.751} $\pm$ 0.005 & 0.735 $\pm$ 0.013 & \textbf{0.736} $\pm$ 0.012 \\
& & & 5  & 0.753 $\pm$ 0.003 & \textbf{0.765} $\pm$ 0.004 & 0.733 $\pm$ 0.011 & \textbf{0.740} $\pm$ 0.013 \\
& & & 7  & 0.762 $\pm$ 0.004 & \textbf{0.784} $\pm$ 0.002 & 0.731 $\pm$ 0.014 & \textbf{0.739} $\pm$ 0.010 \\
& & & 9  & 0.775 $\pm$ 0.005 & \textbf{0.808} $\pm$ 0.003 & \textbf{0.732} $\pm$ 0.012 & 0.728 $\pm$ 0.011 \\
& & & 10 & 0.783 $\pm$ 0.005 & \textbf{0.821} $\pm$ 0.007 & \textbf{0.727} $\pm$ 0.016 & 0.724 $\pm$ 0.019 \\
& & & 20 & 0.885 $\pm$ 0.013 & \textbf{0.972} $\pm$ 0.015 & \textbf{0.702} $\pm$ 0.009 & 0.689 $\pm$ 0.015 \\
& & NN   & -- & 0.744 $\pm$ 0.002 & \textbf{0.748} $\pm$ 0.004 & 0.737 $\pm$ 0.007 & \textbf{0.741} $\pm$ 0.009 \\

\addlinespace

\multirow{7}{*}{} & \multirow{7}{*}{NQ-Open} & \multirow{6}{*}{Tree} & 3  & 0.565 $\pm$ 0.008 & \textbf{0.674} $\pm$ 0.009 & 0.527 $\pm$ 0.011 & \textbf{0.622} $\pm$ 0.051 \\
& & & 5  & 0.596 $\pm$ 0.015 & \textbf{0.745} $\pm$ 0.006 & 0.527 $\pm$ 0.020 & \textbf{0.627} $\pm$ 0.023 \\
& & & 7  & 0.636 $\pm$ 0.019 & \textbf{0.829} $\pm$ 0.009 & 0.508 $\pm$ 0.039 & \textbf{0.627} $\pm$ 0.053 \\
& & & 9  & 0.676 $\pm$ 0.019 & \textbf{0.913} $\pm$ 0.005 & 0.540 $\pm$ 0.030 & \textbf{0.634} $\pm$ 0.047 \\
& & & 10 & 0.697 $\pm$ 0.018 & \textbf{0.944} $\pm$ 0.012 & 0.522 $\pm$ 0.030 & \textbf{0.608} $\pm$ 0.045 \\
& & & 20 & 0.870 $\pm$ 0.024 & \textbf{1.000} $\pm$ 0.000 & 0.519 $\pm$ 0.027 & \textbf{0.621} $\pm$ 0.033 \\
& & NN & -- & 0.535 $\pm$ 0.012 & \textbf{0.593} $\pm$ 0.012 & 0.564 $\pm$ 0.039 & \textbf{0.585} $\pm$ 0.042 \\

\addlinespace

\multirow{7}{*}{} & \multirow{7}{*}{CoQA} & \multirow{6}{*}{Tree} & 3  & 0.665 $\pm$ 0.004 & \textbf{0.672} $\pm$ 0.005 & 0.661 $\pm$ 0.009 & \textbf{0.668} $\pm$ 0.013 \\
& & & 5  & 0.669 $\pm$ 0.003 & \textbf{0.681} $\pm$ 0.005 & 0.659 $\pm$ 0.009 & \textbf{0.661} $\pm$ 0.007 \\
& & & 7  & 0.678 $\pm$ 0.003 & \textbf{0.704} $\pm$ 0.004 & \textbf{0.654} $\pm$ 0.009 & 0.653 $\pm$ 0.012 \\
& & & 9  & 0.693 $\pm$ 0.004 & \textbf{0.737} $\pm$ 0.005 & 0.647 $\pm$ 0.006 & \textbf{0.649} $\pm$ 0.017 \\
& & & 10 & 0.701 $\pm$ 0.003 & \textbf{0.758} $\pm$ 0.008 & 0.640 $\pm$ 0.009 & \textbf{0.644} $\pm$ 0.012 \\
& & & 20 & 0.798 $\pm$ 0.014 & \textbf{0.962} $\pm$ 0.011 & \textbf{0.623} $\pm$ 0.004 & 0.595 $\pm$ 0.010 \\
& & NN & -- & 0.662 $\pm$ 0.003 & \textbf{0.664} $\pm$ 0.003 & 0.661 $\pm$ 0.011 & \textbf{0.662} $\pm$ 0.009 \\

\midrule

\multirow{22}{*}{\textbf{N-gram}} & \multirow{7}{*}{TriviaQA} & \multirow{6}{*}{Tree} & 3  & 0.748 $\pm$ 0.004 & \textbf{0.751} $\pm$ 0.003 & 0.745 $\pm$ 0.015 & \textbf{0.748} $\pm$ 0.012 \\
& & & 5  & 0.754 $\pm$ 0.004 & \textbf{0.765} $\pm$ 0.005 & 0.740 $\pm$ 0.013 & \textbf{0.746} $\pm$ 0.005 \\
& & & 7  & 0.764 $\pm$ 0.003 & \textbf{0.785} $\pm$ 0.003 & 0.734 $\pm$ 0.015 & \textbf{0.742} $\pm$ 0.007 \\
& & & 9  & 0.777 $\pm$ 0.005 & \textbf{0.812} $\pm$ 0.003 & 0.733 $\pm$ 0.012 & \textbf{0.735} $\pm$ 0.007 \\
& & & 10 & 0.786 $\pm$ 0.007 & \textbf{0.826} $\pm$ 0.006 & 0.730 $\pm$ 0.010 & \textbf{0.733} $\pm$ 0.007 \\
& & & 20 & 0.892 $\pm$ 0.020 & \textbf{0.975} $\pm$ 0.013 & \textbf{0.699} $\pm$ 0.002 & 0.694 $\pm$ 0.015 \\
& & NN  & -- & 0.746 $\pm$ 0.003 & \textbf{0.748} $\pm$ 0.005 & 0.745 $\pm$ 0.013 & \textbf{0.750} $\pm$ 0.014 \\

\addlinespace

& \multirow{7}{*}{NQ-Open} & \multirow{6}{*}{Tree} & 3  & 0.566 $\pm$ 0.008 & \textbf{0.661} $\pm$ 0.013 & 0.502 $\pm$ 0.045 & \textbf{0.593} $\pm$ 0.029 \\
& & & 5  & 0.603 $\pm$ 0.017 & \textbf{0.708} $\pm$ 0.016 & 0.521 $\pm$ 0.026 & \textbf{0.610} $\pm$ 0.040 \\
& & & 7  & 0.651 $\pm$ 0.014 & \textbf{0.758} $\pm$ 0.025 & 0.509 $\pm$ 0.035 & \textbf{0.613} $\pm$ 0.031 \\
& & & 9  & 0.688 $\pm$ 0.017 & \textbf{0.815} $\pm$ 0.030 & 0.487 $\pm$ 0.045 & \textbf{0.582} $\pm$ 0.038 \\
& & & 10 & 0.710 $\pm$ 0.019 & \textbf{0.843} $\pm$ 0.032 & 0.505 $\pm$ 0.044 & \textbf{0.581} $\pm$ 0.039 \\
& & & 20 & 0.883 $\pm$ 0.045 & \textbf{0.979} $\pm$ 0.016 & 0.502 $\pm$ 0.048 & \textbf{0.576} $\pm$ 0.038 \\
& & NN  & -- & 0.539 $\pm$ 0.009 & \textbf{0.611} $\pm$ 0.011 & 0.518 $\pm$ 0.022 & \textbf{0.588} $\pm$ 0.031 \\

\addlinespace

& \multirow{7}{*}{CoQA} & \multirow{6}{*}{Tree} & 3  & 0.662 $\pm$ 0.003 & \textbf{0.664} $\pm$ 0.003 & \textbf{0.649} $\pm$ 0.014 & 0.647 $\pm$ 0.011 \\
& & & 5  & 0.668 $\pm$ 0.003 & \textbf{0.677} $\pm$ 0.005 & \textbf{0.645} $\pm$ 0.011 & 0.634 $\pm$ 0.010 \\
& & & 7  & 0.680 $\pm$ 0.004 & \textbf{0.700} $\pm$ 0.007 & \textbf{0.643} $\pm$ 0.012 & 0.640 $\pm$ 0.012 \\
& & & 9  & 0.693 $\pm$ 0.006 & \textbf{0.737} $\pm$ 0.016 & \textbf{0.639} $\pm$ 0.009 & 0.633 $\pm$ 0.018 \\
& & & 10 & 0.701 $\pm$ 0.009 & \textbf{0.759} $\pm$ 0.019 & \textbf{0.640} $\pm$ 0.013 & 0.627 $\pm$ 0.013 \\
& & & 20 & 0.821 $\pm$ 0.023 & \textbf{0.954} $\pm$ 0.019 & \textbf{0.612} $\pm$ 0.013 & 0.589 $\pm$ 0.014 \\
& & NN  & -- & 0.658 $\pm$ 0.003 & \textbf{0.663} $\pm$ 0.004 & 0.653 $\pm$ 0.016 & \textbf{0.660} $\pm$ 0.015 \\


\bottomrule
\end{tabular}
\caption{Accuracy across tree depths, datasets, and feature types. Bold indicates higher accuracy between log-only and full features. Model: RedPajama-INCITE-7B; metric: ROUGE-L.}

\label{tab:classifier-results}
\end{table*}

==> table_7b_rougeL_nostopwords.tex <==
\begin{table*}[!t]
\centering
\small
\begin{tabular}{@{}lllc@{\hskip 6pt}cc|@{\hskip 6pt}cc@{}}
\toprule
\textbf{Feature Type} & \textbf{Dataset} & \textbf{Model} & \textbf{Tree Depth} & \textbf{Train Acc (Log)} & \textbf{Train Acc (Full)} & \textbf{Test Acc (Log)} & \textbf{Test Acc (Full)} \\
\midrule

\multirow{22}{*}{\textbf{Raw Freq}} & \multirow{7}{*}{TriviaQA} & \multirow{6}{*}{Tree}
& 3  & 0.747 $\pm$ 0.003 & \textbf{0.750} $\pm$ 0.005 & 0.735 $\pm$ 0.013 & \textbf{0.738} $\pm$ 0.013 \\
& & & 5  & 0.753 $\pm$ 0.003 & \textbf{0.764} $\pm$ 0.006 & 0.733 $\pm$ 0.011 & \textbf{0.742} $\pm$ 0.011 \\
& & & 7  & 0.762 $\pm$ 0.004 & \textbf{0.785} $\pm$ 0.004 & 0.731 $\pm$ 0.014 & \textbf{0.739} $\pm$ 0.015 \\
& & & 9  & 0.775 $\pm$ 0.005 & \textbf{0.808} $\pm$ 0.005 & \textbf{0.732} $\pm$ 0.012 & 0.730 $\pm$ 0.018 \\
& & & 10 & 0.783 $\pm$ 0.005 & \textbf{0.825} $\pm$ 0.006 & 0.727 $\pm$ 0.016 & \textbf{0.728} $\pm$ 0.022 \\
& & & 20 & 0.885 $\pm$ 0.013 & \textbf{0.981} $\pm$ 0.009 & \textbf{0.702} $\pm$ 0.009 & 0.688 $\pm$ 0.013 \\
& & NN & -- & 0.744 $\pm$ 0.002 & \textbf{0.747} $\pm$ 0.004 & 0.737 $\pm$ 0.007 & \textbf{0.741} $\pm$ 0.009 \\

\addlinespace

& \multirow{7}{*}{NQ-Open} & \multirow{6}{*}{Tree}
& 3  & 0.565 $\pm$ 0.008 & \textbf{0.672} $\pm$ 0.007 & 0.527 $\pm$ 0.011 & \textbf{0.634} $\pm$ 0.053 \\
& & & 5  & 0.596 $\pm$ 0.015 & \textbf{0.735} $\pm$ 0.012 & 0.527 $\pm$ 0.020 & \textbf{0.624} $\pm$ 0.035 \\
& & & 7  & 0.636 $\pm$ 0.019 & \textbf{0.827} $\pm$ 0.005 & 0.508 $\pm$ 0.039 & \textbf{0.629} $\pm$ 0.066 \\
& & & 9  & 0.676 $\pm$ 0.019 & \textbf{0.908} $\pm$ 0.003 & 0.540 $\pm$ 0.030 & \textbf{0.638} $\pm$ 0.031 \\
& & & 10 & 0.697 $\pm$ 0.018 & \textbf{0.935} $\pm$ 0.009 & 0.522 $\pm$ 0.030 & \textbf{0.631} $\pm$ 0.019 \\
& & & 20 & 0.870 $\pm$ 0.024 & \textbf{1.000} $\pm$ 0.000 & 0.519 $\pm$ 0.027 & \textbf{0.617} $\pm$ 0.032 \\
& & NN & -- & 0.535 $\pm$ 0.012 & \textbf{0.591} $\pm$ 0.013 & 0.564 $\pm$ 0.039 & \textbf{0.585} $\pm$ 0.040 \\

\addlinespace

& \multirow{7}{*}{CoQA} & \multirow{6}{*}{Tree}
& 3  & 0.665 $\pm$ 0.004 & \textbf{0.672} $\pm$ 0.005 & 0.661 $\pm$ 0.009 & \textbf{0.668} $\pm$ 0.013 \\
& & & 5  & 0.669 $\pm$ 0.003 & \textbf{0.681} $\pm$ 0.005 & 0.659 $\pm$ 0.009 & \textbf{0.661} $\pm$ 0.007 \\
& & & 7  & 0.678 $\pm$ 0.003 & \textbf{0.705} $\pm$ 0.005 & 0.654 $\pm$ 0.009 & \textbf{0.656} $\pm$ 0.011 \\
& & & 9  & 0.693 $\pm$ 0.004 & \textbf{0.737} $\pm$ 0.008 & \textbf{0.647} $\pm$ 0.006 & 0.645 $\pm$ 0.012 \\
& & & 10 & 0.701 $\pm$ 0.003 & \textbf{0.757} $\pm$ 0.010 & 0.640 $\pm$ 0.009 & \textbf{0.642} $\pm$ 0.009 \\
& & & 20 & 0.798 $\pm$ 0.014 & \textbf{0.954} $\pm$ 0.015 & \textbf{0.623} $\pm$ 0.004 & 0.595 $\pm$ 0.017 \\
& & NN & -- & 0.662 $\pm$ 0.003 & \textbf{0.664} $\pm$ 0.003 & 0.661 $\pm$ 0.011 & 0.661 $\pm$ 0.010 \\

\midrule

\multirow{22}{*}{\textbf{N-gram}} & \multirow{7}{*}{TriviaQA} & \multirow{6}{*}{Tree}
& 3  & 0.748 $\pm$ 0.004 & \textbf{0.751} $\pm$ 0.003 & 0.745 $\pm$ 0.015 & \textbf{0.748} $\pm$ 0.012 \\
& & & 5  & 0.754 $\pm$ 0.004 & \textbf{0.764} $\pm$ 0.004 & 0.740 $\pm$ 0.013 & \textbf{0.747} $\pm$ 0.009 \\
& & & 7  & 0.764 $\pm$ 0.003 & \textbf{0.786} $\pm$ 0.004 & 0.734 $\pm$ 0.015 & \textbf{0.744} $\pm$ 0.017 \\
& & & 9  & 0.777 $\pm$ 0.005 & \textbf{0.811} $\pm$ 0.008 & 0.733 $\pm$ 0.012 & \textbf{0.734} $\pm$ 0.015 \\
& & & 10 & 0.786 $\pm$ 0.007 & \textbf{0.828} $\pm$ 0.007 & \textbf{0.730} $\pm$ 0.010 & 0.723 $\pm$ 0.011 \\
& & & 20 & 0.892 $\pm$ 0.020 & \textbf{0.970} $\pm$ 0.010 & \textbf{0.699} $\pm$ 0.002 & 0.685 $\pm$ 0.005 \\
& & NN & -- & 0.746 $\pm$ 0.003 & \textbf{0.749} $\pm$ 0.004 & 0.745 $\pm$ 0.013 & \textbf{0.746} $\pm$ 0.014 \\

\addlinespace

& \multirow{7}{*}{NQ-Open} & \multirow{6}{*}{Tree}
& 3  & 0.566 $\pm$ 0.008 & \textbf{0.665} $\pm$ 0.012 & 0.502 $\pm$ 0.045 & \textbf{0.590} $\pm$ 0.016 \\
& & & 5  & 0.603 $\pm$ 0.017 & \textbf{0.704} $\pm$ 0.017 & 0.521 $\pm$ 0.026 & \textbf{0.605} $\pm$ 0.030 \\
& & & 7  & 0.651 $\pm$ 0.014 & \textbf{0.775} $\pm$ 0.018 & 0.509 $\pm$ 0.035 & \textbf{0.606} $\pm$ 0.023 \\
& & & 9  & 0.688 $\pm$ 0.017 & \textbf{0.841} $\pm$ 0.019 & 0.487 $\pm$ 0.045 & \textbf{0.578} $\pm$ 0.023 \\
& & & 10 & 0.710 $\pm$ 0.019 & \textbf{0.869} $\pm$ 0.023 & 0.505 $\pm$ 0.044 & \textbf{0.587} $\pm$ 0.022 \\
& & & 20 & 0.883 $\pm$ 0.045 & \textbf{0.990} $\pm$ 0.019 & 0.502 $\pm$ 0.048 & \textbf{0.570} $\pm$ 0.033 \\
& & NN & -- & 0.539 $\pm$ 0.009 & \textbf{0.612} $\pm$ 0.014 & 0.518 $\pm$ 0.022 & \textbf{0.581} $\pm$ 0.028 \\

\addlinespace

& \multirow{7}{*}{CoQA} & \multirow{6}{*}{Tree}
& 3  & 0.662 $\pm$ 0.003 & \textbf{0.664} $\pm$ 0.003 & \textbf{0.649} $\pm$ 0.014 & 0.647 $\pm$ 0.011 \\
& & & 5  & 0.668 $\pm$ 0.003 & \textbf{0.678} $\pm$ 0.006 & \textbf{0.645} $\pm$ 0.011 & 0.635 $\pm$ 0.012 \\
& & & 7  & 0.680 $\pm$ 0.004 & \textbf{0.702} $\pm$ 0.007 & \textbf{0.643} $\pm$ 0.012 & 0.642 $\pm$ 0.016 \\
& & & 9  & 0.693 $\pm$ 0.006 & \textbf{0.740} $\pm$ 0.007 & \textbf{0.639} $\pm$ 0.009 & 0.628 $\pm$ 0.020 \\
& & & 10 & 0.701 $\pm$ 0.009 & \textbf{0.763} $\pm$ 0.013 & \textbf{0.640} $\pm$ 0.013 & 0.625 $\pm$ 0.020 \\
& & & 20 & 0.821 $\pm$ 0.023 & \textbf{0.958} $\pm$ 0.025 & \textbf{0.612} $\pm$ 0.013 & 0.581 $\pm$ 0.017 \\
& & NN & -- & 0.658 $\pm$ 0.003 & \textbf{0.663} $\pm$ 0.005 & 0.653 $\pm$ 0.016 & \textbf{0.661} $\pm$ 0.017 \\

\bottomrule
\end{tabular}
\caption{Accuracy across tree depths, datasets, and feature types, with stopwords filtered from occurrence features. Bold indicates higher accuracy between log-only and full features. Model: RedPajama-INCITE-7B; metric: ROUGE-L.}

\label{tab:classifier-results-nostopwords}
\end{table*}

==> table_7b_rougeL_short.tex <==
\begin{table*}[!t]
\centering
\small
\begin{tabular}{@{}lllc@{\hskip 6pt}cc|@{\hskip 6pt}cc@{}}
\toprule
\textbf{Feature Type} & \textbf{Dataset} & \textbf{Model} & \textbf{Tree Depth} & \textbf{Train Acc (Log)} & \textbf{Train Acc (Full)} & \textbf{Test Acc (Log)} & \textbf{Test Acc (Full)} \\
\midrule

\multirow{11}{*}{\textbf{Raw Freq}} & \multirow{3}{*}{TriviaQA} & \multirow{2}{*}{Tree} & 3  & 0.747 $\pm$ 0.003 & \textbf{0.751} $\pm$ 0.005 & 0.735 $\pm$ 0.013 & \textbf{0.736} $\pm$ 0.012 \\
& & & 7  & 0.762 $\pm$ 0.004 & \textbf{0.784} $\pm$ 0.002 & 0.731 $\pm$ 0.014 & \textbf{0.739} $\pm$ 0.010 \\
& & NN   & -- & 0.744 $\pm$ 0.002 & \textbf{0.748} $\pm$ 0.004 & 0.737 $\pm$ 0.007 & \textbf{0.741} $\pm$ 0.009 \\

\addlinespace

\multirow{7}{*}{} & \multirow{3}{*}{NQ-Open} & \multirow{2}{*}{Tree} & 3  & 0.565 $\pm$ 0.008 & \textbf{0.674} $\pm$ 0.009 & 0.527 $\pm$ 0.011 & \textbf{0.622} $\pm$ 0.051 \\
& & & 7  & 0.636 $\pm$ 0.019 & \textbf{0.829} $\pm$ 0.009 & 0.508 $\pm$ 0.039 & \textbf{0.627} $\pm$ 0.053 \\
& & NN & -- & 0.535 $\pm$ 0.012 & \textbf{0.593} $\pm$ 0.012 & 0.564 $\pm$ 0.039 & \textbf{0.585} $\pm$ 0.042 \\

\addlinespace

\multirow{7}{*}{} & \multirow{3}{*}{CoQA} & \multirow{2}{*}{Tree} & 3  & 0.665 $\pm$ 0.004 & \textbf{0.672} $\pm$ 0.005 & 0.661 $\pm$ 0.009 & \textbf{0.668} $\pm$ 0.013 \\
& & & 7  & 0.678 $\pm$ 0.003 & \textbf{0.704} $\pm$ 0.004 & \textbf{0.654} $\pm$ 0.009 & 0.653 $\pm$ 0.012 \\
& & NN & -- & 0.662 $\pm$ 0.003 & \textbf{0.664} $\pm$ 0.003 & 0.661 $\pm$ 0.011 & \textbf{0.662} $\pm$ 0.009 \\

\midrule

\multirow{11}{*}{\textbf{N-gram}} & \multirow{3}{*}{TriviaQA} & \multirow{2}{*}{Tree} & 3  & 0.748 $\pm$ 0.004 & \textbf{0.751} $\pm$ 0.003 & 0.745 $\pm$ 0.015 & \textbf{0.748} $\pm$ 0.012 \\
& & & 7  & 0.764 $\pm$ 0.003 & \textbf{0.785} $\pm$ 0.003 & 0.734 $\pm$ 0.015 & \textbf{0.742} $\pm$ 0.007 \\
& & NN  & -- & 0.746 $\pm$ 0.003 & \textbf{0.748} $\pm$ 0.005 & 0.745 $\pm$ 0.013 & \textbf{0.750} $\pm$ 0.014 \\

\addlinespace

& \multirow{3}{*}{NQ-Open} & \multirow{2}{*}{Tree} & 3  & 0.566 $\pm$ 0.008 & \textbf{0.661} $\pm$ 0.013 & 0.502 $\pm$ 0.045 & \textbf{0.593} $\pm$ 0.029 \\
& & & 7  & 0.651 $\pm$ 0.014 & \textbf{0.758} $\pm$ 0.025 & 0.509 $\pm$ 0.035 & \textbf{0.613} $\pm$ 0.031 \\
& & NN  & -- & 0.539 $\pm$ 0.009 & \textbf{0.611} $\pm$ 0.011 & 0.518 $\pm$ 0.022 & \textbf{0.588} $\pm$ 0.031 \\

\addlinespace

& \multirow{3}{*}{CoQA} & \multirow{2}{*}{Tree} & 3  & 0.662 $\pm$ 0.003 & \textbf{0.664} $\pm$ 0.003 & \textbf{0.649} $\pm$ 0.014 & 0.647 $\pm$ 0.011 \\
& & & 7  & 0.680 $\pm$ 0.004 & \textbf{0.700} $\pm$ 0.007 & \textbf{0.643} $\pm$ 0.012 & 0.640 $\pm$ 0.012 \\
& & NN  & -- & 0.658 $\pm$ 0.003 & \textbf{0.663} $\pm$ 0.004 & 0.653 $\pm$ 0.016 & \textbf{0.660} $\pm$ 0.015 \\


\bottomrule
\end{tabular}
\caption{Classifier accuracy across tree depths, datasets, and feature types. Bold indicates the higher value between log-only and full feature sets for each row. Note: in the $n$-gram results, generations shorter than $n$ tokens are excluded, so the test set for $n$-gram features is a subset of the raw frequency setting.}

\label{tab:classifier-results-short}
\end{table*}
